Approximating Values of Generalized-Reachability Stochastic Games

Simple stochastic games are turn-based 2.5-player games with a reachability objective. The basic question asks whether one player can ensure reaching a given target with at least a given probability. A natural extension is games with a conjunction of such conditions as objective. Despite a plethora of recent results on the analysis of systems with multiple objectives, the decidability of this basic problem remains open. In this paper, we present an algorithm approximating the Pareto frontier of the achievable values to a given precision. Moreover, it is an anytime algorithm, meaning it can be stopped at any time returning the current approximation and its error bound.

==> 5_stepBoundProof.tex <==


\section{Step bound for $\epsilon$-approximating lower value iteration}

\todo{add transition to this sec}
\todo{finish the proof}

We know from \cite{cfk13} that executing value iteration for k iterations computes the pareto curve for k-step bounded reachability.
We prove in Theorem 1 that there exists a bound $\bound$, such that the $\bound$-step pareto curve is $\epsilon$-close to all achievable points.
This then implies that running VI for $\bound$ steps correctly computes an $\epsilon$-approximation of the achievable points. 
$\bound$ is exponential in $\states$, logarithmic in $\epsilon$, linear in $m$ and something with $\actmin$ that we do not know yet.
\todo{Make sure that this is the same definition of $\epsilon$-approximation we use everywhere in the paper.}

\begin{theorem}
	For any SG $\G$ with $m$ target sets and for all $\epsilon>0$, it holds for every achievable point $\vec{x}$ that $\vec{x} - \vec\epsilon$ is in the $\bound$-step Pareto frontier, where $\bound = m * \abs{\states} * \frac {\log(\epsilon)}{\log(1-(\transmin\cdot \actmin)^{\abs{\states<?>}})}$, where $\transmin$ is the minimal transition probability in $\G$ and $\actmin$ is the minimal probability that a \todogeneric{smart $\epsilon$-optimal strategy uses}.
\end{theorem}
\begin{proof}
	
	We proceed by induction on the number of targets.	
	
	\begin{itemize}
		\item [Base Case:] Let $m=1$. 
		Note that deterministic strategies suffice for unbounded and step-bounded reachability in SGs~\cite{condonComplexity}; for the latter, assume we unfold the game with a step counter and then do unbounded reachability in the unfolded game; then it can use memory (the step counter), but still is deterministic.
		Hence we can assume that the minimal probability any strategy uses is $\actmin = 1$.
		
		For states in the target set $T$ or states with value 0, called sinks $\sink \eqdef \set{\state \in \states \mid V(\state) = 0}$, we are done after the initialization, as states with value 0 have the correct value, and states in $T$ are correctly set to 1.
		So we only need to consider the remaining states $\states<?> \eqdef \states \setminus (T \cup \sink)$.
		
		Let $\sigma$ be a $k$-step optimal strategy of Maximizer, with $k \geq \abs{\states}$. 
		Then, for all $\state \in \states<?>$ and all deterministic Minimizer counter-strategies there exists a path from $\state$ to $T$ in $\G[\sigma,\tau]$.
		This is the case, because $V(\state)>0$ as it is in $\states<?>$, so Maximizer can ensure that the state reaches the target, and there must be a cycle-free path of length at most $\abs{\states}$; since we use a strategy that is optimal for at least $\abs{\states}$ steps, this path or something even better has to be used by $\sigma$.
		It is not a problem to restrict to deterministic counter-strategies, as these are optimal.
		
		Since the strategies are deterministic, the probability of the path is at least $x \eqdef (\actmin*\transmin)^{\abs{\states}} = \transmin[\abs{\states}]$ (Equality holds as $\actmin=1$ as argued above).
		
		Let $i = \floor{k / \abs{\states}}$ be the number of $\abs{\states}$-step phases that the $k$-step optimal strategy we picked considers.
		In each of these phases, the probability to reach $T$ is at least $x$.
		The remaining probability is split between staying in $\states<?>$ and going to $\sink$. 
		In the next phase, the states in $\sink$ have no chance to reach $T$ any more, while the ones in $\states<?>$ again have a probability of $x$.
		Thus, after $i$ phases, the probability to reach either $T$ or $\sink$ from any $\state \in \states<?>$ is at least $\sum_{j=1}^{i} x * (1-x)^j$; every summand is the minimum probability to not reach for $j-1$ phases and then reach in the $j$-th phase. If probability goes to the sinks, that only increases the probability to reach $T$ or $\sink$.
		To arrive at an $\epsilon$-optimal value, we need to find an $i$ such that $\sum_{j=1}^{i} x * (1-x)^j \geq 1 - \epsilon$.
		Using the closed form of the sum, this simplifies to $1 - (1-x)^i \geq 1 - \epsilon$; by reformulating, we get $i \geq \frac {\log(\epsilon)}{\log(1-x)}$.
		So, after $i = \frac{\log(\epsilon)}{\log(1-x)}$ phases, the probability to reach either the targets or sinks is at least $1-\epsilon$. 
		An $i$-phase ($i*\abs{\states}$-step) optimal strategy will distribute the probability mass of at least $1-\epsilon$ optimally between $T$ and $\sink$, and thus be $\epsilon$-close to the true value.
		%Thus, by running value iteration for$i*\abs{\states}$ steps, we get an $\epsilon$-approximation of the value, because VI computes the step bounded value correctly and we just proved that it is $\epsilon$-close to the true value.
		
		The step bound is an instantiation of the one postulated in the theorem, with $m$ and $\actmin$ equal to 1.
		
		
		
		\item [Induction Hypothesis:] For any SG $\G$ with $m$ targets and for all $\epsilon>0$, it holds for every achievable point $\vec{x}$ that $\vec{x} - (\epsilon,\dots,\epsilon)$ is in the $\bound$-step pareto curve, where $\bound = m * \abs{\states} * \frac {\log(\epsilon)}{\log(1-(\transmin\cdot \actmin)^{\abs{\states<?>}})}$.
		
		\item [Induction Step:]
		Now we assume we have $m+1$ targets. 
		By an argument similar to the base case, we prove below that the number of steps necessary to find an $\epsilon$-optimal strategy for reaching the union of all target sets or the sink states is $\abs{\states} * \frac {\log(\epsilon)}{\log(1-(\transmin\cdot \actmin)^{\abs{\states<?>}})}$; in the sink states we are done, as the value is correctly 0; after reaching a target set, we can consider the simplified game with only $m$ targets and apply the induction hypothesis to estimate the number of steps remaining as $m * \abs{\states} * \frac {\log(\epsilon)}{\log(1-(\transmin\cdot \actmin)^{\abs{\states<?>}})} $.
		Thus, we get the required result that the total number of steps is at most $(m+1) * \abs{\states} * \frac {\log(\epsilon)}{\log(1-(\transmin\cdot \actmin)^{\abs{\states<?>}})}$.
		
		Note that we are $\epsilon$-close to the best value for the first target that we reach. 
		This holds for all targets, proving that we are at most substracting $\epsilon$ in all dimensions. \todo{check that this really is true, more formal} => In fact not true, instead we have to distribute our $\epsilon$ among the targets. Each target gets $\epsilon / m$ prob that it may not distribute. Then overall only $\epsilon$ is unassigned.
		
		There are two things that change in comparison to the proof in the base case.
		
		Firstly, we need to prove that there for every point on the k-step  Pareto curve ($k\geq\abs{\states}$), there exists a k-step optimal strategy $\sigma$ to achieve this point that "makes progress". "Making progress" is defined as follows: For all counter strategies $\tau$, all path-lengths that are smaller than $k - \abs{\states}$ and all states $\state \in \states<?>$, 
		in $\G[\sigma,\tau]$ there exists a path of length at most $\abs{\states}$ with positive probability from $\state$ to $\bigcup_{i \in [1, m]} T_i$.
		Intuitively this means, that, as long as the strategy still knows what to do, so path length less than $k$, it will never run around in an EC; instead, it will always have a plan to reach some target within the next $\abs{\states}$ steps. 
		To prove this, we show that any running around in ECs can be replaced by using randomization.
		
		Secondly, we need to prove that there is a lower bound on the probability that the strategy assigns to any action, namely $\actmin$. 
		
		When these two things work, we can use the analogue of the base case, using $x \eqdef (\transmin\cdot \actmin)^{\abs{\states<?>}}$, as now the strategy could randomize putting only $\actmin$ on progressing in each step. 
		
	\end{itemize}
	
	
\end{proof}

\todo{this is collection of thoughts on the proof}
Write Lemma 1 and 2 formulation.
Try to prove Lemma 1

Lemma 1: In arbitrary unfolded SG, memoryless strats suffice in ECs.
There can't be in an EC with target in it.
If I'm locked in, strat doesn't matter.
Otherwise I am S? and want to reach something, I need to leave. Want some distribution over exits.

Consider the regions of the eps-approx curve: In every region, it is clear how I want to leave, so for every point memless det suffices.


See whiteboard:
It is in general not true that states in an EC have the same value in a MOSG.
Tobis CE to det strat: Not possible to get both states to the same value for anything but trivial cases (0,0) (0,1) or (1,0).





fix arb strat for 1 player
this is eps approx

consider T step reach
it will become eps approx of the arb strat

so pick eps approx, then play for T steps to become eps close
now we have 2eps-close strat


Small change in strat only changes values a little

After having Lemma 1, everything becomes transient and Lemma 2 should be easy.


Lemma 1:
In goal-unfolded game, in ECs, memoryless strategies suffice for eps-optimal value.
(This implies the Lemma 1 that we formulated in draft)

proof idea: In every regional SEC, min cooperates, so there we have MR, cause in MO-MDP we have MR.
Use the regions of the eps-approx curve (which exists, since DEC by converging algo)


==> 7_proofs.tex <==
\section{Technical details of the proofs}\label{sec:proofs}

\todo{add proofs for the Lemmata from Sec 4; update section structure, fix refs from section 4 to be more precise}

\subsection{Soundness}\label{sec:proofsa}


\begin{lemma}[$\GETREGIONS$ is sound and correct]\label{lem:getRegionscorr}
For any set of states $T$ and bound function $\lb$, the set of regions $\mathcal{R}$ returned by getRegions($T,\lb$) has the following properties:
\begin{enumerate}
\item $\biguplus_{R \in \mathcal{R}} R = \directions$
\item For each $R \in \mathcal{R}$, for all directions $\dir \in \directions$ the relative order of exits is the same. More formally: 
$\forall \dir_1,\dir_2 \in R, \state<1>,\state<2> \in T_\Box, i \in \set{1,2}, \action<i> \in \Av(\state<i>), (\state<i>,\action<i>) \leaves T:$\\
\hspace*{-1em}$\lb(\state<1>,\action<1>)[\dir_1] \geq \lb(\state<2>,\action<2>)[\dir_1] \implies \lb(\state<1>,\action<1>)[\dir_2] \geq \lb(\state<2>,\action<2>)[\dir_2].$
\end{enumerate}
\end{lemma}
\begin{proof}
That $\bigcup \mathcal R=\directions$ follows easily from the initialization to the whole $\directions$ and staying within this cone.
Disjointness follows from the definition of SC, which ensures that self-interiors of any its two elements either do not intersect or equal one of them.
For the second claim, consider directions $\dir_1,\dir_2$ such that $\lb(\state<1>,\action<1>)[\dir_1] \geq \lb(\state<2>,\action<2>)[\dir_1]$, but $\lb(\state<1>,\action<1>)[\dir_2] < \lb(\state<2>,\action<2>)[\dir_2]$.
If the former inequality is strict, then the two directions are split by an intersection of the frontiers of $\lb(\state<1>,\action<1>)$ and $\lb(\state<2>,\action<2>)$.
The intersection then splits also the projection and thus also the produced SC and hence also the regions.
If instead equality holds, then one of the directions is on the boundary.
However, the boundary is then projected and turned into a face of the SC, hence into a simplex, whose parts are turned into regions.
In either case, $\dir_1$ and $\dir_2$ lie in different regions.
\end{proof}


\begin{lemma}[$\FINDSECS$ is sound and correct, given well formed regions]\label{lem:FINDSECS}
For $T \subseteq \states$, a lower bound function $\lb$ and a region $R$, where the relative ordering of exits is the same for all directions in $R$, it holds that $X \in \FINDSECS(T,\Av,\lb,R) \iff X$ is an inclusion maximal $\rSEC$ with respect to $\lb$.
\end{lemma}
\begin{proof}
If a direction $\dir$ is fixed, $\lb(\state)[\dir] \in \Reals$. 
The proof of \cite[Lemma 2]{cav18} works directly. 
We now argue that this is the case for all $\dir \in R$. 
Given that the relative ordering of exits is same for all $\dir \in R$, for any two actions $\action<1>$ and $\action<2>$ $\lb(\state, \action<1>)[\dir_1] \geq \lb(\state, \action<2>)[\dir_1] \implies \lb(\state, \action<1>)[\dir_2] \geq \lb(\state, \action<2>)[\dir_2]$. 
This implies that $\set{\action \in \Av(s) \mid \lb(\state, \action)[\dir] > \lb(\state)[\dir]}$ is the same for all $\dir \in R$. 
Consequently, the set $B$ computed on line \ref{alg:findsecs:B} of the $\FINDSECS$ procedure is the same for all $\dir \in R$. 
Hence, \cite[Lemma 2]{cav18} immediately proves this lemma once any random $\dir \in R$ is chosen.
\end{proof}



\todo{thoroughly type check the whole paper. Find\_SECs sometimes has a G, sometimes not}


%We never use this; it is just something we probably want to have
%\begin{lemma}[$\doSECs$ is dwc and convex]\label{lem:deflateMonDwcConv}
%For any set of states $T \subseteq \states$ and upper and lower bound functions $\ub$ and $\lb$, it holds that after executing $\MODEFLATE(\lb,\ub,T)$ $\ub[\prime]$ is dwc and convex for each state.
%\end{lemma}
%\begin{proof}
%Dwc and convex: Massaging in the end ensures this.
%\end{proof}

%\begin{lemma}[$\doSECs$ is Scott-continuous]\label{lem:do-secs-continuous}
%For any directed chain $\set{(\lb<1>, \ub<1>), (\lb<2>, \ub<2>), \dots}$
%\end{lemma}

\subsection{Convergence}\label{sec:proofsb}

\begin{lemma}[Continuity] \label{lem:cont}
$\mop$ is Scott-continuous. \todo{hard to get proof right, possibly doesn't even hold, we do not need it anymore because we decided to show directed that limit of operator is also a fixpoint}
\end{lemma}
\begin{proof}
$\mop$ operates on the domain $\mathcal{D} = {(\Reals^{n})}^{\states \cup \states \times \actions}$.
We write $\mathbf b = (\lb, \ub) \in \mathcal{D}$ to denote an element in this domain.
We define a partial order on $\mathcal D$ and write $\mathbf b_1 \leq \mathbf b_2$ if $\mathbf b_1$ is component-wise ``worse'' than $\mathbf b_2$, i.e. $\lb<1> \leq \lb<2>$ and $\ub<1> \geq \lb<2>$.
A directed chain $D \in \mathcal{D}$ is denoted as $\set{(\lb<1>, \ub<1>), (\lb<2>, \ub<2>), \dots}$.
In order to show Scott-continuity, we need to show that for every directed chain $D$, $\sqcup (\mop (D)) = \mop (\sqcup (D))$ (where $\sqcup$ is the meet).
\cite[Proposition 8]{DBLP:journals/iandc/BassetKW18} shows that $\bellman$ is Scott-continuous.
Lemmata \ref{lem:do-secs-sound} and \ref{lem:do-secs-monotonic} show that $\DEFLATE$ is monotonic and order-preserving. \todot{monotonic=order-pres?}
Hence, $\mop$ is monotonic and order-preserving and consequently it follows that $\sqcup (\mop (D)) = \mop (\sqcup (D))$.
\end{proof}

\begin{proof}[Proof of Fact 2]\todo{improve, explain bottom MEC, maybe use ideas from journal? somewhere there is a typo where we use U instead of Uinf. Explain the problems why we need Z and Y does not suffice, or scratch the whole buisness, or move to appendix. Add what being a MEC in X means (i.e. being a MEC and being subseteq of X).}
We have the context of the proof of Proposition 3, in particular we know that $X \subseteq \states$ contains an EC and that for all states $\state \in X: \Delta(\state) = \max_{\state \in \states} \Delta(\state)=\dif$.
\begin{enumerate}
\item Let $X' \subseteq X$ be a bottom MEC in $X$.
	\paragraph*{Justification}
	We compute the MEC decomposition of $X$ and pick a MEC at the end of a chain. 
	$X'$ exists, since there is an EC in $X$, so there also is at least one MEC in $X$.
\item Let $m = \max_{\state \in X'} \ub(\state)[\dir]$ be the maximal upper bound in $X'$.
\item Let $Y := \set{\state \mid \state \in X' \wedge \ub(\state)[\dir] =m}$ be the states with maximal upper bound in $X'$.
\item $\forall \state \in Y, \exists \action \in \Av(\state): \neg (\state,\action) \leaves Y$, i.e. all states in $Y$ have actions that stay in $Y$. \label{step:stayY}
	\paragraph*{Reasoning}
	\begin{enumerate}
	\item If for some state $\state \in Y$ all available actions left $X$, it would have to depend on the outside of $X$, and by Fact 1 this is a contradiction.
	Thus $\state$ has actions that stay in $X$.
	\item No action can exit from $Y$ to $X \setminus X'$, because $X'$ is a bottom MEC in $X$. \label{step:XsetminusX'}
	If an action left to some state $t \in X \setminus X'$, then, since $X'$ is a bottom MEC in $X$, from $t$ there would be no reachable EC in $X$. 
	Starting from $t$, this is the same situation as when $X$ does not contain an EC, and thus Fact 1 yields a contradiction.
	\item Not all actions can exit to $X' \setminus Y$. 
	$\ub(\state) = m$ and for every $\state[\prime] \in X' \setminus Y: \ub(\state[\prime])[\dir] < m$.
	So if the action exits $Y$ to $X'$, the upper bound of the action is smaller than $m$, since part of the successors have a smaller upper bound.
	It cannot have another successor with a higher upper bound, because it has to stay in $X'$, and $m$ is chosen to be the highest upper bound in $X'$.
	There has to be some action with upper bound $m$, because $\ub(\state)[\dir] = m$. 
	Thus, not all actions can leave to $X'$.
	\item Aggregating the previous points:
	Not all actions can exit $X$, no action can exit to $X \setminus X'$, not all actions can exit to $X' \setminus Y$. So some action has to remain in $Y$.
	\end{enumerate}
\item Let $Z$ be a bottom MEC in $Y$.
	\paragraph*{Justification}
	We compute the MEC decomposition of $X$ and pick a MEC at the end of a chain. 
	$Z$ exists, since by the previous step there must exists an EC in $Y$, since all states have staying actions.
\item For all states $\state \in Z: \val(\state)[\dir] = m - \dif$.
	\paragraph*{Justification}
	Since $Z \subseteq Y$, $\ub<\infty>(\state)[\dir] = m$
	Since $Y \subseteq X$, $\Delta(\state) = \dif$.
	We get the following chain of equations:
	$\dif = \Delta(\state) = \ub<\infty>(\state)[\dir] - \val(\state)[\dir] = m - \val(\state)[\dir]$
	Reordering yields the statement.
\item Thus, $Z$ is an $\rSEC$ for region $\set{\dir}$.
\item When applying $\mop$ once more, $Z \in \mathcal{S}$ in Line \ref{line:find} of Algorithm \ref{alg:doSECs}. \label{step:isFound}
	\paragraph*{Reasoning}
	$X' \in MEC(\G)$ by definition of $X'$.
	So $\mathcal{R} \gets \GETREGIONS(X',\lb<\infty>)$ is executed. 
	Since $\biguplus_{R \in \mathcal{R}} R = \mathcal{D}$ by Lemma \ref{lem:getRegionscorr}, there is some $R \in \mathcal{R}$ with $\dir \in R$.
	Also by that Lemma we have that the relative order of exits for all directions in $R$ is the same, and since it was called with $\lb<\infty>$, it is correct. 
	Thus, we can apply Lemma \ref{lem:FINDSECS}, which proves the statement.
\item $\cas(Z)[\dir] < m$ \label{step:smaller}
	\paragraph*{Reasoning}
	$\cas(Z)[\dir]$ must put positive weight on some exit of $Z$. If it puts positive weight on some state-action-pair that exits $X$, then by Fact 1 $\cas(Z)[\dir] < m$.
	The only other possible exit is to $X' \setminus Y$. 
	This is because of the fact the $Z$ is a bottom MEC in $Y$ and the argumentation in Step \ref{step:stayY}.
	For all states $\state' \in X' \setminus Y$, it holds that $\ub(\state')[\dir] < m$.
	If $\cas(Z)[\dir]$ is constructed from a convex combination of exits only to $X' \setminus Y$, then also $\cas(Z)[\dir]< m$.
\item $\forall \state \in Z: \mop(\ub<\infty>)(\state)[\dir] = \cas(Z)[\dir]$
	\paragraph*{Reasoning}
	Let $\state \in Z$.
	The upper bound is modified by only Line \ref{line:actualDeflate}.
	Since $\dir \in R$ by how the algorithm found $Z$ (Step \ref{step:isFound}) and since $\cas(Z)[\dir] < m = \ub(\state)[\dir]$, the new upper bound is exactly $\cas(Z)[\dir]$ for each $\state \in Z$.
\item Thus, by combining the previous two steps, we finally arrive at a contradiction, 
since $\forall \state \in Z: \mop(\ub<\infty>)(\state)[\dir] = \cas(Z)[\dir] < \ub<\infty>(\state)[\dir]$

\end{enumerate}
\end{proof}










\iffalse
%This claim 1 is not strong enough. I keep it here so we can see what the proof of the new claim 1 should look like.
%Since it might be renamed: It is the part of the proof that says that you may not depend on the outside.
\textbf{Claim 1:} No state in $X$ may depend on a leaving action. Unnegated: Every state in $X$ may only depend on staying actions.
		$\forall (\state,\action) \in \exits(X_\circ): \val(\state)[\dir] < \val(\state,\action)[\dir]$ as well as
		$\forall (\state,\action) \in \exits(X_\Box): \ub(\state)[\dir] > \ub(\state,\action)[\dir]$.
		
\paragraph*{Proof of Claim 1}
We assume $X := \set{\state \mid \state \in \states \wedge \Delta(\state) = \max_{\state \in \states} \Delta(\state)}$. 
\begin{enumerate}
\item Pick some $(\state,\action) \leaves X$. Then there exists a $t \in \post(\state,\action) \setminus X$, with $\Delta(t) < \Delta(\state)$.
\item \begin{align*}
	\ub<\infty>(\state,\action)[\dir] &= \delta(\state,\action,t) \cdot \ub<\infty>(t)[\dir] \\
		&+ \sum_{\state[\prime] \in \Av(\state)\setminus\set{t}} \delta(\state,\action,\state[\prime]) \cdot \ub<\infty>(\state[\prime])[\dir]\\
	\val(\state,\action)[\dir] &= \delta(\state,\action,t) \cdot \val(t)[\dir] \\
		&+ \sum_{\state[\prime] \in \Av(\state)\setminus\set{t}} \delta(\state,\action,\state[\prime]) \cdot \val(\state[\prime])[\dir]
	\end{align*}
	so it follows that
	\begin{align*}
	\Delta(\state,\action) &= \delta(\state,\action,t) \cdot \Delta(t)\\
		&+ \sum_{\state[\prime] \in \Av(\state)\setminus\set{t}} \delta(\state,\action,\state[\prime]) \cdot \Delta(\state[\prime])\\
		&< \Delta(\state)\tag{Since $\Delta(t) < \Delta(\state)$ and $\Delta(\state[\prime] \leq \Delta(\state)$ by definition of $X$}
	\end{align*}
\item $\val(\state)[\dir] - \val(\state,\action))[\dir] < \ub<\infty>(\state))[\dir] - \ub<\infty>(\state,\action))[\dir]$, by applying the definition of $\Delta$ to the previous inequation and reordering.\label{step:ineq}
\item We now derive the claim by a case distinction over the player of $\state$.
	\begin{itemize}
	\item[Case $\state \in X_\circ$:]
	Then, $\ub<\infty>(\state,\action))[\dir] \geq \ub<\infty>(\state)[\dir]$ from $\state$ being a Minimizer state. 
	Using this in the equation from Step \ref{step:ineq} yields $\val(\state)[\dir] - \val(\state,\action))[\dir] < 0$, or by reordering
	$\val(\state)[\dir] <\val(\state,\action))[\dir]$, which is the first part of the claim.
	\item[Case $\state \in X_\Box$:]
	Then $\val(\state)[\dir] \leq \val(\state,\action)[\dir]$. 
	Using this in the equation from Step \ref{step:ineq} yields $\ub<\infty>(\state)[\dir] - \ub<\infty>(\state,\action))[\dir] > 0$, or by reordering
	$\ub<\infty>(\state)[\dir] > \ub<\infty>(\state,\action)[\dir]$.
	\end{itemize}
	
\end{enumerate}


%Case X does not contain an EC
%	We invert the definition of EC.  
%	We get that for all non-empty $B \subseteq \bigcup_{\state \in X} \Av(\state)$ one of two things hold:
%	\begin{itemize}
%	\item There exists an $\state<\ell> \in X, \action<\ell> \in B$ such that $(\state<\ell>,\action<\ell>) \leaves X$. 
%	\item There exist $\state<1>,\state<2> \in X$, such that for all finite paths from $\state<1>$ to $\state<2>$ it holds that they are not in $(X \times B)* \times X$, i.e. they leave $X$ or or use actions not in $B$.
%	\end{itemize}
%	\todo{Somehow, from this it follows} that some state only has leaving actions available. Thus this state obviously depends on something outside of $X$, and by Claim 1, we are done.

\item It holds that $(\state,\action) \leaves Z \implies (\state,\action) \leaves X$. %Only for Z_circ, and we do not need it anymore
	\paragraph*{Reasoning}
	By Step \ref{step:XsetminusX'}, no action can exit from $Z$ to $X \setminus X'$, and by applying the same argumentation, we get that no action can exit from $Z$ to $Y \setminus Z$.
	It remains to show that actions exiting to $X' \setminus Y$ are also not possible. 
\fi


